Can Automated Feedback Turn Students into Happy Prologians?

Providing personalized feedback is essential for effective learning, but delivering it promptly can be challenging in large-scale courses. In this work, we present ProHelp, an automated assessment platform for Prolog built on top of the GitSeed framework, and we evaluate it through a survey of 144 students from a 365-student undergraduate logic programming course. We assessed the perceived usefulness of seven types of automated feedback, including automatic testing, predicate scoring, syntax error highlighting, open choice point warnings, score rankings, solution type validation, and unknown predicate name suggestions. Our results show that 74% of students agreed the feedback helped increase their grade, and the system achieved a System Usability Scale score of 78.5 (grade B+). Among the feedback types, automatic testing was ranked as the most useful, followed by open choice point warnings and predicate scoring, with statistically significant differences. We found no significant effect of students' interest level, engagement with optional exercises, or use of large language models on their perception of feedback usefulness. We also explore student preferences for future feedback features, finding a significant preference for showing the differences between generated and expected test outputs.

==> eptcsdata.tex <==
\providecommand{\firstpage}{179}
\providecommand{\publicationstatus}{W. Faber, L. Giordano, R. Rocha, V. Santos Costa (Eds.):\\ 42nd International Conference on Logic Programming (ICLP 2026)\\
EPTCS 450, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.450.15}{10.4204/EPTCS.450.15}}
\pdfoutput=1

